Sort-free Gaussian Splatting via Weighted Sum Rendering

Recently, 3D Gaussian Splatting (3DGS) has emerged as a significant advancement in 3D scene reconstruction, attracting considerable attention due to its ability to recover high-fidelity details while maintaining low complexity. Despite the promising results achieved by 3DGS, its rendering performance is constrained by its dependence on costly non-commutative alpha-blending operations. These operations mandate complex view dependent sorting operations that introduce computational overhead, especially on the resource-constrained platforms such as mobile phones. In this paper, we propose Weighted Sum Rendering, which approximates alpha blending with weighted sums, thereby removing the need for sorting. This simplifies implementation, delivers superior performance, and eliminates the "popping" artifacts caused by sorting. Experimental results show that optimizing a generalized Gaussian splatting formulation to the new differentiable rendering yields competitive image quality. The method was implemented and tested in a mobile device GPU, achieving on average $1.23\times$ faster rendering.

==> rebuttal/rebuttal.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  All reviewers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Weaknesses}

We thank reviewers for their constructive and thoughtful comments, which has significantly enhanced the quality of our submission. Below, we provide general comments, followed by specific responses to each reviewer's remarks.

Summary of Common Strengths and Weaknesses

Strengths:
\begin{itemize}
    \item The paper is well-motivated, addressing a critical bottleneck in 3D Gaussian Splatting (3DGS) rendering by introducing a sort-free pipeline. 
    \item  The proposed learnable weighted sum rendering technique as well as view dependent opacity offer substantial performance improvements.
    \item The performance gains are particularly notable on mobile devices.
    \item The method effectively mitigates "pop" artifacts, a persistent challenge in volumetric rendering. 
\end{itemize}


Weakness:
\begin{itemize}
    \item The paper requires a comparison with methods that reduce the number of Gaussians and with 3DGS implementations in WebGL.
    \item The theoretical foundation needs further justification.
    \item The analysis of memory usage and GPU resource exhaustion needs clarification.
\end{itemize}

As a general comment, in this paper we consider the fact that for Gaussian Splatting to be successfully used in mobile devices, it should not only be rendered in real time, but also with low power usage. While many works aim to reduce complexity, our focus is specifically on addressing the sorting problem.


% We have shared videos created with WSR at https:..., including specific tests requested by the reviewers. They show the quality of the new view synthesis in general. The reviewers can observe some artifacts, but it should be considered that some are caused by the training loss function, which is averaging over views, and may appear to converge when there are still some low quality outliers that can be fixed with additional iterations. This is currently under investigation.

% As a general comment, in this paper we consider the fact that for Gaussian Splatting to be successfully used in mobile devices, it should not only be rendered in real time, but also with low power usage. There are many works aiming to reduce complexity, but our paper is focused on the sorting problem. The proposed solution can be combined with other methods, but that would greatly complicate the analysis and would not fit in a single conference paper.

% As mentioned by reviewer ``Man9,'' higher performance may also be achieved with new GPU hardware specialized for 3DGS, but that is uncertain, costly, and may take many years. 

% Our paper is about how to use the hardware acceleration that is already in mobile GPUs and evaluate its effectiveness. We believe this will is the type of information that is essential to decide if new hardware is needed, and what type. In fact, sorting and tiling are very bad for parallelization, which means it is much easier to design efficient specialized hardware when there is no sorting.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  First Reviewer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Reviewer 1: ``FZe3''}

\subsection{Weaknesses}

% The proposed method gets rid of the costly sorting, but a more complex weight and view-dependent opacity are used. Although the author points out in the paper that a general scheme for learning scene representations is bound only by the mathematical constraints of the scene model. According to the experimental results in the paper, the use of simple weighted-sum and view-independent opacity cannot achieve satisfactory rendering results. Does this mean that for rendering processes that are not physically and optically, more complex models must be used, such as introducing more learnable parameters as in the paper?

% \amir{We believe there are two meanings for the word ``complexity'' that are related to this observation. Our proposal indeed adds more spherical harmonic parameters, and from a human perspective can appear more ``complex'' in the sense of complicated. However, for efficient GPU implementation memory use has to be aligned by powers of two, so color data is represented as RGBARGBA... instead of RBGRGB... We exploit this fact by using the alpha memory position to create view-dependent opacity, and the result is that what we propose actually does not increase the amount of memory and vector operations, i.e., computational complexity.}

% \reply{It's tricky problem. Simple WSR and view-independent opacity would lead to incorrect rendering for the occluded areas. To alleviate the problem, we introduced more parameters to model the transparency. For the learnable parameters, traditional OIT heriously designed weight functions, which is able to achieve reasonable performance.  In our paper, we show that learnable parameters would further improve the quality of synthesized image in Table . It's a complex question, we have smaller numbers of Gaussians.}


% \reply{RGBA in graphic pipeline, we always need to calculate the RGBA even in the 3dgs, where calculate RGB. It's in the training, in the testing time, all parameters are fixed. }


% \amir{Moving away from physical and optical intuition can also appear to make it more complicated, but it is becoming common in machine learning to discover that non-intuitive approaches can be computationally more effective. View-dependent opacity would not make sense in a physically-based model, but WSR is different from that. Thus, it should not be interpreted strictly as opacity, but mathematically as a term in a model reproducing radiance fields.}


\officialquestion{Rendering rendering processes that are not physically and optically, more complex models must be used, such as introducing more learnable parameters?}


\officialreply{We recognize that the term "complexity" can be interpreted in two distinct ways in this context. Our proposal introduces additional spherical harmonic parameters, which may appear more "complex" or complicated from a human perspective. However, our method actually reduces computational complexity and requires less memory compared to 3D Gaussian Splatting (3DGS), as demonstrated in Tables 2 and 3 of our paper. First, our method eliminates the sorting step. Second, the data in GPU graphic pipeline is represented as RGBARGBA$\cdots$ instead of RBGRGB$\cdots$ We exploit this fact by using the alpha memory position to create view-dependent opacity, which does not increase the amount of memory and vector operations, i.e., computational complexity.}



% In the conclusion part of the paper, the author mentioned some recent research on compact Gaussian Splatting. According to my understanding of these works, since the methods proposed in these works obtain more compact 3D Gaussian representations, they can reduce the sorting overhead and speed up rendering to a certain extent. Therefore, I think the author should add a comparison of rendering quality, speed and memory usage between the proposed method and these works, such as Compact 3DGS[1], LightGaussian[2] and Compressed 3DGS[3] in the experimental evaluation section.


% \reply {Thank you for your suggestion. We updated Table~1 as well as the experiment section to compare rendering quality with Compact 3DGS, LightGaussian, and Compressed 3DGS. We need to discuss the speed and memory. We compare our method on the Vulkan implementation. These methods, however, are based on the CUDA. These methods can not utilize the graphic pipeline, which would significantly slow down their }


\officialquestion{Compare with Compact 3DGS, LightGaussian, and Compressed 3DGS}


\officialreply{Thank you for your suggestion. We updated Table 1 as well as the experiment section to compare rendering quality with Compact 3DGS, LightGaussian, and Compressed 3DGS. We also updated the Tables in the supplementary materials to include the results for each scene. For speed and memory comparisons, we evaluated our method on mobile devices. However, the aforementioned methods are implemented using CUDA, and many features, such as codebooks, are not supported in the mobile GPU graphics pipeline. Consequently, we were unable to perform a direct comparison within the limited time.}

\begin{table}
    \setlength{\tabcolsep}{3.5pt}
    \centering
    \footnotesize
    % \tiny
    % \fontsize{7}{10}\selectfont
    \caption{PSNR scores of our method on the Mip-NeRF360 dataset, the Tanks \& Temples dataset, and the Deep Blending dataset. Our method achieved comparable results with 3DGS.} \label{table:rst} \vspace{-0.in}
    \begin{tabular}{lccccccccc}
    % {P{2.1cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}}
        \toprule
        \multirow{2}[2]{*}{Method} & \multicolumn{3}{c}{Mip-NeRF 360} & \multicolumn{3}{c}{Tanks \& Temples} & \multicolumn{3}{c}{Deep Blending}  
        \\ \cmidrule(lr){2-4}  \cmidrule(lr){5-7}  \cmidrule(lr){8-10} 
         &PSNR↑ &SSIM↑ &LPIPS↓ &PSNR↑ &SSIM↑ &LPIPS↓ &PSNR↑ &SSIM↑ &LPIPS↓
        \\ \midrule
        Plenoxels & 23.08 & 0.626 & 0.463 & 21.08 & 0.719 & 0.379 & 23.06 & 0.795 & 0.510 \\ 
        INGP-Base  & 25.30 & 0.671 & 0.371 & 21.72 & 0.723 & 0.330 & 23.62 & 0.797 & 0.423 \\ 
        INGP-Big  & 25.59 & 0.699 & 0.331 & 21.92 & 0.745 & 0.305 & 24.96 & 0.817 & 0.390 \\ 
        M-NeRF360  & \textbf{27.69} & 0.792 & 0.237 & 22.22 & 0.759 & 0.257 & 29.40 & 0.901 & 0.245 \\ 
        3DGS  & 27.21 & \textbf{0.815} & 0.214 & 23.14 & 0.841 & 0.183 & 29.41 & \textbf{0.903} & 0.243 \\ 
        Compact 3DGS  & 27.08 & 0.798 & 0.247 & \textbf{23.71} & 0.831 & 0.178 & \textbf{29.79} & 0.901 & 0.258 \\
        LightGaussian & 27.28 & 0.805 & 0.243  & 23.11 & 0.817 & 0.231  & - & - & - \\
        Compressed 3DGS & 26.98 & 0.801 & 0.238 & 23.32 & 0.832 & 0.194 & 29.38 & 0.898 & 0.253 \\
        \midrule
        LC-WSR & 27.19 & 0.804 & \textbf{0.211} & 23.61 & \textbf{0.842} & \textbf{0.177} & 29.63 & 0.902 & \textbf{0.229} \\
        \bottomrule
    \end{tabular}\vspace{-0.in}   
\end{table}


\begin{table}
\setlength{\tabcolsep}{1.5pt}
    \centering
    % \footnotesize
    % \tiny
    \fontsize{7}{10}\selectfont
    \caption{PSNR scores of our method on the Mip-NeRF360 dataset, the Tanks\&Temples dataset, and the Deep Blending dataset.} \label{table:comp_psnr} \vspace{-0.in}
    \begin{tabular}{ccccccccccccccccc}
    % {P{2.1cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}}
        \toprule
        \multirow{2}[2]{*}{Method} & \multicolumn{10}{c}{Mip-NeRF360} & \multicolumn{3}{c}{Tanks\&Temples} & \multicolumn{3}{c}{Deep Blending}  
        \\ \cmidrule(lr){2-11}  \cmidrule(lr){12-14}  \cmidrule(lr){15-17} 
         &bicycle &flowers &garden &stump &treehill &room &counter &kitchen &bonsai &Avg  &truck &train &Avg &drjohnson &playroom &Avg 
        \\ \midrule
        
        Plenoxels &21.91 &20.10 &23.49 &20.66 &22.25 &27.59 &23.62 &23.42 &24.67 &23.08 &23.22 &18.93 &21.08 &23.14 &22.98 &23.06  \\
        INGP-Base &22.19 &20.35 &24.60 &23.63 &22.36 &29.27 &26.44 &28.55 &30.34 &25.30 &23.26 &20.17 &21.72 &27.75 &19.48 &23.62  \\
        INGP-Big &22.17 &20.65 &25.07 &23.47 &22.37 &29.69 &26.69 &29.48 &30.69 &25.59 &23.38 &20.46 &21.92 &28.26 &21.67 &24.96  \\
        Mip-NeRF360 &24.31 &\textbf{21.65} &26.88 &26.18 &\textbf{22.93} &31.47 &29.45 &\textbf{31.99} &\textbf{33.40} &\textbf{27.69} &24.91 &19.52 &22.22 &29.14 &29.66 &29.40  \\
        3DGS &\textbf{25.25} &21.52 &27.41 &\textbf{26.55} &22.49 &30.63 &28.70 &30.32 &31.98 &27.21 &25.18 &21.09 &23.14 &28.77 &\textbf{30.04} &29.41  \\
        Compact 3DGS &24.77 &20.89 &26.81 &26.46 &22.65 &30.88 &28.71 &30.48 &32.08 &27.08 &25.35 &22.07 &23.71 &29.06 &29.87 &29.46\\
        Compressed 3DGS &24.97 &21.15 &26.75 &26.29 &22.26 &31.14 &28.67 &30.26 &31.35 &26.98 &24.82 &21.86 &23.34 &28.87 &29.89 &29.38 \\
        LightGaussian & 25.20 & 21.54 & 26.96 & 26.77 & 22.69 & 31.40 & 28.48 & 30.87 & 31.41 &27.13 & \textbf{25.40} & 21.84 & 23.44 & - & - & - \\
        \midrule
        % Ours-v15 &24.02 &20.48 &26.96 &24.83 &21.37 &30.77 &28.67 &30.15 &31.13 &24.1 &21.21 &29.12 &29.36  \\
        % Ours-v17 &23.64 &19.42 &27.20 &24.43 &21.48 &31.43 &29.43 &30.94 &32.53 &24.32 &21.56 &29.10 &29.72 \\
        Ours-LC &24.20 & 20.45 & \textbf{27.78} & 25.39 & 22.01 & \textbf{31.93} & \textbf{29.53} & 31.38 & 32.05 & 27.19 & 25.28 & \textbf{21.93} & \textbf{23.61} & \textbf{29.25} & 30.00 & \textbf{29.63} \\
        \bottomrule
    \end{tabular}\vspace{-0.in}   
\end{table}





\begin{table}
\setlength{\tabcolsep}{1.5pt}
    \centering
    % \footnotesize
    % \tiny
    \fontsize{7}{10}\selectfont
    \caption{SSIM scores of our method on the Mip-NeRF360 dataset, the Tanks\&Temples dataset, and the Deep Blending dataset.} \label{table:comp_ssim} \vspace{-0.in}
    \begin{tabular}{ccccccccccccccccc}
    % {P{2.1cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}}
        \toprule
        \multirow{2}[2]{*}{Method} & \multicolumn{10}{c}{Mip-NeRF360} & \multicolumn{3}{c}{Tanks\&Temples} & \multicolumn{3}{c}{Deep Blending}  
        \\ \cmidrule(lr){2-11}  \cmidrule(lr){12-14}  \cmidrule(lr){15-17} 
         &bicycle &flowers &garden &stump &treehill &room &counter &kitchen &bonsai &Avg  &truck &train &Avg &drjohnson &playroom &Avg 
        \\ \midrule
        
        Plenoxels & 0.496 & 0.431 & 0.606 & 0.523 & 0.509 & 0.8417 & 0.759 & 0.648 & 0.814 & 0.626 & 0.774 & 0.663 & 0.719 & 0.787 & 0.802 & 0.795 \\
        INGP-Base & 0.491 & 0.450 & 0.649 & 0.574 & 0.518 & 0.855 & 0.798 & 0.818 & 0.890 & 0.671  & 0.779 & 0.666  & 0.723 & 0.839 & 0.754 & 0.797 \\
        INGP-Big & 0.512 & 0.486 & 0.701 & 0.594 & 0.542 & 0.871 & 0.817 & 0.858 & 0.906  & 0.699   & 0.800 & 0.689 & 0.745 & 0.854 & 0.779   & 0.817 \\
        Mip-NeRF360 & 0.685 & 0.583 & 0.813 & 0.744 & 0.632 & 0.913 & 0.894 & 0.920 & \textbf{0.941} & 0.792  & 0.857 & 0.660 & 0.759 & \textbf{0.901} & 0.900  & 0.901 \\
        3DGS & \textbf{0.771} & \textbf{0.605} & 0.868 & 0.775 & \textbf{0.638} & 0.914 & 0.905 & 0.922 & 0.938  & \textbf{0.815}  & 0.879 & \textbf{0.802} & 0.841 & 0.899 & \textbf{0.906} & \textbf{0.903} \\
        Compact 3DGS &0.723 &0.556 &0.832 &0.757 &0.638 &0.919 &0.902 &0.919 &0.939 &0.798 &0.871 &0.792  &0.831 &0.900 &0.902 &0.901 \\
        Compressed 3DGS &0.751 &0.584 &0.844 & 0.757 &0.620  &0.896 & 0.914 & \textbf{0.914} & 0.930  &0.801 &0.867  &0.798 &0.832 &0.895 &0.900 &0.898 \\
        LightGaussian & 0.765 & 0.598 & 0.855 & \textbf{0.776} & 0.635 & 0.916 & 0.898 & 0.919 & 0.934 & 0.806 & 0.877 & 0.801 & 0.832 & - & - & -\\
        \midrule
        Ours & 0.744 & 0.580 & \textbf{0.872} & 0.728 & 0.614 & \textbf{0.925} & 0.909 & \textbf{0.923} & 0.938 & 0.804 & \textbf{0.882} & \textbf{0.802} & \textbf{0.842} & 0.898 & \textbf{0.906} & 0.902  \\
        \bottomrule
    \end{tabular}\vspace{-0.in}   
\end{table}


\begin{table}
\setlength{\tabcolsep}{1.5pt}
    \centering
    % \footnotesize
    % \tiny
    \fontsize{7}{10}\selectfont
    \caption{LPIPS scores of our method on the Mip-NeRF360 dataset, the Tanks\&Temples dataset, and the Deep Blending dataset. } \label{table:comp_lpips} \vspace{-0.in}
    \begin{tabular}{ccccccccccccccccc}
    % {P{2.1cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}P{0.45cm}}
        \toprule
        \multirow{2}[2]{*}{Method} & \multicolumn{10}{c}{Mip-NeRF360} & \multicolumn{3}{c}{Tanks\&Temples} & \multicolumn{3}{c}{Deep Blending}  
        \\ \cmidrule(lr){2-11}  \cmidrule(lr){12-14}  \cmidrule(lr){15-17} 
         &bicycle &flowers &garden &stump &treehill &room &counter &kitchen &bonsai &Avg  &truck &train &Avg &drjohnson &playroom &Avg 
        \\ \midrule
        
        Plenoxels & 0.506 & 0.521 & 0.386 & 0.503 & 0.540 & 0.4186 & 0.441 & 0.447 & 0.398 & 0.463 & 0.335 & 0.422 & 0.379 & 0.521 & 0.499 & 0.510 \\
        INGP-Base & 0.487 & 0.481 & 0.312 & 0.450 & 0.489 & 0.301 & 0.342 & 0.254 & 0.227 & 0.371  & 0.274 & 0.386  & 0.330 & 0.381 & 0.465 & 0.423 \\
        INGP-Big & 0.446 & 0.441 & 0.257 & 0.421 & 0.450 & 0.261 & 0.306 & 0.195 & 0.205 & 0.331   & 0.249 & 0.360  &  0.305 & 0.352 & 0.428   & 0.390 \\
        Mip-NeRF360 & 0.301 & 0.344 & 0.170 & 0.261 & 0.339 & 0.211 & 0.204 & 0.127 & 0.176 & 0.237  & 0.159 & 0.354  & 0.257 & 0.237 & 0.252  & 0.245 \\
        3DGS & \textbf{0.205} & \textbf{0.336} & 0.103 & \textbf{0.210} & 0.317 & 0.220 & 0.204 & 0.129 & 0.205 & 0.214  & 0.148 & \textbf{0.218}  & 0.183 & 0.244 & 0.241 & 0.243 \\
        Compact 3DGS & 0.286 & 0.399 & 0.161 & 0.278 & 0.363 & 0.209 & 0.205 & 0.131 & 0.193 & 0.247 & 0.163 & 0.240 & 0.201 & 0.258 & 0.258 & 0.258 \\
        Compressed 3DGS & 0.240 & 0.358 &  0.144 & 0.250  &  0.351 & 0.231 & 0.215 & 0.140  & 0.217 & 0.238 & 0.161 & 0.226 & 0.194 & 0.254 & 0.252 & 0.253 \\
        LightGaussian & 0.218 & 0.352 & 0.122 & 0.222 & 0.338 & 0.232 & 0.220 & 0.141 & 0.221 & 0.237 & 0.155 & 0.239 & 0.202 & - & - & - \\
        \midrule
        % Ours-v15 &24.02 &20.48 &26.96 &24.83 &21.37 &30.77 &28.67 &30.15 &31.13 &24.1 &21.21 &29.12 &29.36  \\
        % Ours-v17 &23.64 &19.42 &27.20 &24.43 &21.48 &31.43 &29.43 &30.94 &32.53 &24.32 &21.56 &29.10 &29.72 \\
        Ours & \textbf{0.205} & 0.342 & \textbf{0.097} & 0.235 & \textbf{0.311} & \textbf{0.197} & \textbf{0.191} & \textbf{0.125} & \textbf{0.199} & \textbf{0.211} & \textbf{0.136} & 0.219 & \textbf{0.177} & \textbf{0.233} & \textbf{0.225} & \textbf{0.229} \\
        \bottomrule
    \end{tabular}\vspace{-0.in}   
\end{table}



\subsection{Questions}
% In the paper, the author points out that for some complex scenes, since a large number of 3D Gaussians are needed for representation, the sorting process will exhaust the resources of mobile devices, making real-time rendering impossible, such as the bicycle scene in Mip-NeRF 360 dataset. However, I tried to visualize the bicycle scene using a gsplat-based webgl viewer on my phone (iPhone 15 Pro Max), and was surprised to find that it achieves real-time rendering, about 20-30fps. This seems to indicate that some optimizations to the 3DGS rendering pipeline (gsplat uses some tricks) can increase the rendering speed on mobile devices without more complex designs. I would like to know the author's opinion on my point of view and more analyses of the key differences that enable real-time performance on mobile devices. And they can test the performance of gsplat on Snapdragon® 8gen3 chipset and compare with their proposed method.

% Here is the link of gsplat webgl-viewer https://gsplat.tech

% \reply{\qiqi{Randall. Zifeng} Resolution 1024 * 768, ours is 1920 * 1080. For the gsplat.tech website, it will further reduce the resolution by 2 times once it is detected on the mobile devices. It seems that the bicycle is 115Mb, much smaller than the official gs around 1.5G. They also reduce the number of Gaussian from 6127390 to . In their implementation, their SH degree is set to 0. we conduct the experiments to run our methods under the same setting, including reducing the resolution to 1024 * 768, reduce the color sh to 0. Our method speed up the rendering significantly from \textbf{**} fps to \textbf{**} fps on a Snapdragon 8 gen 3 chips. These improvement can be attributed to the leverage of graphic pipeline in GPU as well as the . We also need to analyse the bottleneck. We also compare the speed ours with webGL on the bicycle scenes

% \randall{The gsplat implementation appears to be running at a significantly lower resolution and leverages an asynchronous CPU sort running at a frequency below the framerate, which exacerbates temporally artifacts under motion. Our implementation does not have these artifacts, and can implemented without the added complexity of marshaling data between the CPU and GPU.}
% }

% \qiqi{Compare with other implementation. Not an apple to apple comparison, WebGL: CPU+GPU, ours are purely GPU. Current market don't support hardware only for Gaussians. }

% \qiqi{The author of gsplat.tech also claim that  "WebGL can't do efficient GPU sorting of the splats, so I had to pull some tricks to make it work. The splats are sorted on the CPU and the ordering may take a few frames to get updated on the GPU." only a few frames, the sorting is updated. }



\officialquestion{Compared with gssplat webgl https://gsplat.tech}


\officialreply{Thank you for highlighting this implementation. We conducted the suggested experiment and observed that, at the same rendering resolution, our method improves the rendering speed from 19-25 fps to 30 fps on a Snapdragon 8 Gen 3. The gsplat implementation operates at a significantly lower resolution and utilizes an asynchronous CPU sort running at a frequency below the framerate, which exacerbates temporal artifacts during motion. Our implementation does not exhibit these artifacts. We have included a discussion of these findings in the revised paper. \qiqi{New paragraphy}Furthermore, as noted at the bottom of gsplat.tech, the author acknowledges that sorting is a bottleneck: "There's artifacts when I turn the model quickly. WebGL can't do efficient GPU sorting of the splats, so I had to pull some tricks to make it work. The splats are sorted on the CPU and the ordering may take a few frames to get updated on the GPU."}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Second Reviewer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Reviewer 2: ``Man9''}

\subsection{Weaknesses}
% The theoretical foundation for replacing alpha blending with an algebraic function requires stronger justification. While the proposed representation achieves good results, it lacks the physical insights inherent in traditional alpha blending, which models light obstruction during propagation. The introduction of view-dependent opacity appears necessary for acceptable rendering quality, but the paper would benefit from a more rigorous analysis of why this combination works, rather than empirical validation alone.



% \reply{I need draw more insights from previous works. Order Independent Transparency has a long history in the computer graphics. }

% \reply{\amir{This observation is applicable to most of new ML-based techniques, where rigorous theoretical justifications are missing, but practical results are very good. Similarly, our main objective was not to provide more insight, but to study how mathematical formulations that enable faster computations can effectively substitute physically-based representations.}

% \amir{From this perspective, the addition of view-dependent opacity adds degrees of freedom to enable better solution, but it was motivated by the intuition that WSR needs better control over transparency. With 3DGS the directions within objects are not important, but need to be better controlled with WSR.} }

\officialquestion{The theoretical foundation of the algebraic rendering function requires stronger justification.}


\officialreply{Our paper is inspired by the Order Independent Transparency, which is a traditional rendering method. Our method can be considered as an extension of weighted order-independent blending[1] on Gaussian Splatting.  Our main objective was not to provide more insight, but to study how mathematical formulations that enable faster computations can effectively substitute physically-based representations. From this perspective, the addition of view-dependent opacity adds degrees of freedom to enable better solution, but it was motivated by the intuition that WSR needs better control over transparency. Following your suggestion, we have updated the related work section to establish stronger connections between our work and previous rendering methods.}

[1] McGuire, Morgan, and Louis Bavoil. "Weighted blended order-independent transparency." Journal of Computer Graphics Techniques 2.4 (2013).


% The preference for linear weights over exponential weights raises questions about robustness. When considering camera movement along viewing rays, exponential weights (with $\beta = 1$) should theoretically provide more consistent mixing ratios between Gaussians. Linear weights may introduce color shift artifacts due to distance-dependent mixing ratio variations. While the authors claims "some artifacts remain visible" then selected linear weight rather than exponential weight, these issues warrant more detailed examination.

% \reply{\amir{The opacity factors are applied equally to the RGB color components, so per color consistency is maintained with both weight formulation.}

% \amir{At the same time, it is correct to assume that the combination ratios of different splats are maintained along the z-direction with exponential weights, but not with linear. However, for the test views it is the function that (surprisingly for us) yields the best PSNR results, and visually it is also very good. To demonstrate that we provide a video with camera moving along the z-direction, with a comparison of results using exponential and linear weights.} }


% \reply{\qiqi{I will create a video moving along the z direction}}



\officialquestion{Moving camera along $z$ direction might introduce the color-shifting artifacts}


\officialreply{The alpha and weights are applied equally to the RGB color components. As shown in Eq 7, our method includes a final normalization stage. We agree with reviewer that ratios of different splats are maintained along the z-direction with Exponential Weighted Sum Rendering (EXP-WSR), but not with Linear Correction Weighted Sum Rendering (LC-WSR). However, LC-WSR also produces visually plausible results. We conducted the suggested experiments by moving the camera along the z-direction and tested our EXP-WSR and LC-WSR on the Bicycle and Garden scenes. In the video, we don't observe the color shifting artifacts. We have included a discussion of these findings in the revised paper. The video can be accessed at:: \url{https://anonymous20241121.github.io/sort_free_gs/z_dir.mp4}}










% The method's generalizability is limited by the transformation of opacity into a view-dependent "black box" variable. This fundamentally alters the role of opacity, which traditionally serves as a crucial signal for pruning and densification in many 3DGS applications, potentially limiting compatibility with existing and future research in this domain.

% \amir{The 3DGS densification technique was maintained for WSR training without any modification, while pruning just have to be extended to take an array of values for its decisions. Since we did not observe any degradation in the training, we do not expect compatibility problems.}

% \reply{We agree the authors that current }




\officialquestion{View dependent opacity potentially limits the compatibility with research in pruning and densification.}


\officialreply{The 3DGS densification technique was maintained for our method without any modification, while pruning needs to be extended. We agree with the reviewer that view-dependent opacity is not compatible with some recent densification and pruning methods. However, there are researches exploring other signals, such as mask[2], color[3], for densification and pruning, , which have shown promising results. Our method will benefit from these works in the future.We have included a discussion of this in the revised paper.}

% [1] Lee, Joo Chan, et al. "Compact 3d gaussian representation for radiance field." Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. 2024.
% [2] Bulò, Samuel Rota, Lorenzo Porzi, and Peter Kontschieder. "Revising densification in gaussian splatting." arXiv preprint arXiv:2404.06109 (2024).





\subsection{Questions}
% Does the method exhibit color shift artifacts during camera movement along the z-direction, as suggested by the concerns regarding linear weighting?

% \reply{\qiqi{Videos}}




% Since opacity is not capped at 1, how did you enforce the data range of final color, simply clamp?

% \amir{WSR is defined as a quotient, with opacity and color contributions appearing in the nominator and denominator, and has a final normalization stage. Thus values larger than 1 do not create the problems that would occur with alpha blending, and there is no need to clamp opacity or color values.}

% \reply{WSR contains a normalization term. As shown in Eq 8, the weighted sum rendering will be normalized by the sum of weight. Our final rendered image will be clamped following 3DGS.}



\officialquestion{Since opacity is not capped at 1, how did you enforce the data range of final color, simply clamp?}


\officialreply{Weighted Sum Rendering (WSR) is defined as a quotient, with alpha and weight contributions appearing in the numerator and denominator, followed by a final normalization stage, as shown in Eq 7. Additionally, our final rendered image is clamped in accordance with the 3D Gaussian Splatting (3DGS) method.}





% How do other Gaussian attributes maintain their geometric meaning in this framework? Specifically: Does the mean of Gaussians still correspond to point cloud locations? How about depth extraction?

% \reply{Other Gaussian attributes remains the same as the 3DGS. $xyz$ still indicate the location of Gaussians. In our method, we extracted the same depth from 3DGS, which is used for sorting in 3DGS.}



\officialquestion{How do other Gaussian attributes maintain their geometric meaning in this framework? Specifically: Does the mean of Gaussians still correspond to point cloud locations? How about depth extraction?}


\officialreply{Other Gaussian attributes remain the same as in 3DGS. The $xyz$ coordinates still indicate the location of the Gaussians. In our method, we extract the same depth from 3DGS, which is used for sorting in 3DGS.}




% While traditional 3DGS implementations employ culling to manage computational complexity, does this approach require weighted summation of ALL Gaussians? What are the implications for scalability?

% \amir{The culling stage is exactly the same. Only visible splats need to be added.}



\officialquestion{What about the culling in WSR? }


\officialreply{Culling operates the same as 3DGS. As with 3DGS, we render only those Gaussians within the Camera Frustum. Our implementation does sum over all visible Gaussians, we configure the hardware to perform this summation efficiently using hardware supported blending operations. We added a discussion in the revised paper.}








% Please clarify the memory usage analysis: does it encompass only Gaussian attributes or include runtime memory requirements? What is the memory overhead of spherical harmonics coefficients for view-dependent opacity compared to vanilla 3DGS?

% \reply{Thank you for your suggestion. We compare the runtime memory in Table 3. We have updated our paper to make it clear. For the storage size, our model takes more memory due to the extra spherical harmonics coefficients for view dependent opacity. In our implementation, we extend color spherical harmonics from 16 * 3 (RGB) to 16 * 4 (RGBO). }

% \amir{Please see reply to reviewer ``uk93'': while there is increased external memory, we and other researchers found that spherical harmonic coefficients are the easiest to compress and prune.}



\officialquestion{Clarify the memory usage analysis.}


\officialreply{We compare the runtime memory in Table 3. For view-dependent opacity, the spherical harmonics data in the GPU graphics pipeline is represented as RGBARGBA$\cdots$ instead of RBGRGB$\cdots$. We exploit this by using the alpha memory position to create view-dependent opacity, which does not increase the runtime memory. However, our model requires more storage due to the additional spherical harmonics coefficients for view-dependent opacity. We have updated the caption of Table 3 and the corresponding section in the experiment part of the paper.}



% Regarding Table 2, could you elaborate on the starred data points showing significantly higher values? How does resource exhaustion due to sorting impact subsequent pipeline stages?

% \reply{\qiqi{We need Randall and Zifeng to answer this question.} , cash system. hardware limitation. }



\officialquestion{Why does resource exhaustion lead to significantly higher values?}


\officialreply{Our implementation of 3DGS appears to be hitting some sort of GPU bottleneck when rendering scenes with a large number of sorted Gaussians. Unfortunately, it can be difficult to pinpoint the sources of inefficiency in complex GPUs. To the best of our knowledge, this is caused by sudden changes to many more cache misses.  We suspect that this bottleneck could be addressed with in-depth analysis and GPU specific optimizations, however, this would make our reference implementation less faithful to the original 3DGS implementation. We note that our method appears to avoid this bottleneck in its simplicity. We added a comment about this to the paper.}


% Given the potential for hardware-accelerated sorting methods specifically designed for 3DGS, possibly through hardware-software co-design, how might this work adapt to or complement such future developments?

% \reply{\qiqi{we need  Randall and Zifeng to answer this question.} we have already used the graphic pipeline in GPUs, not specifically. }

% \reply{\randall{There will be no hardware accelerated sorting for 3DGS. There is nothing special about Gaussian Splatting sorting that would differentiate it from a general sorting routine. Optimized sorts are their own area of investigation and interest, any may benefit from optimizations that target various architectures.
% The time-delay from architecting and designing a chip to shipping is 3 years, Gaussian Splatting is currently a 1 year old technique and undergoing heavy research and evolution. If we had already co-designed a chip to optimize GS we could see how that turns out in 2027. A key feature of our technique is that there is no reason it couldn't run on a GPU that is 10 years old.
% The reviewer doesn't know what he is talking about and has asked a dumb question [don't print that].}}

% \reply{linear is the limit whatever algorithm. }


\officialquestion{Given the potential for hardware-accelerated sorting methods specifically designed for 3DGS, possibly through hardware-software co-design, how might this work adapt to or complement such future developments?}



\officialreply{A significant advantage of our technique is its independence from the latest hardware, making it portable to older, lower-power devices and implementable in legacy APIs such as WebGL. The typical time delay from chip design to market release is approximately three years. Given that Gaussian Splatting is a relatively new technique, only one year old and still undergoing extensive research and development, it is expected that future hardware, particularly state-of-the-art and task-specific 3DGS hardware, will surpass our technique in various aspects. However, our method's compatibility with existing, less advanced hardware remains a notable strength.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Third Reviewer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Reviewer 3: ``b3oc''}

% \subsection{Weaknesses}
% ** Motivation **

% As shown in the paper, the sorting step is usually considered slow, but actually contributes to only 25\% of the total rendering time. The real problem preventing 3DGS based method from matching the rendering speed of traditional methods is the alpha blending step. Although this paper removes the sorting step, it still needs the per-pixel alpha blending of Gaussians of calculated weights. As a result, the speed improvement is rather insignificant.
% Rather than removing the sorting step, many works have proposed to removing the redundant Gaussians directly. These methods seem to provide much more significant speed boost. Of course these two method can be run in parallel, but it still weaken the importance of the proposed method.

% \amir{We believe the results may be interesting for graphics specialist considering the fact that low-power GPU rendering can only be achieved with increasingly more efficient parallelization. Sorting is intrinsically sequential, and thus greatly complicates the hardware parallelization by requiring techniques like tiling, and to remove the ``popping'' requires significantly more complicated sorting. Weighted sums, on the other hand, eliminates dependencies and only require atomic add (or vector add) support for parallelization.}

% \reply{\randall{There are many such optimization that are possible in a compute-based API such as CUDA running on an A6000 GPU consuming 300Watts. Our technique can be implemented with any graphics API and run on a phone consuming single digit watts. [too snarky]}}


\officialquestion{Sorting contributes to only 25\% of the total rendering time, while reducing the redundant Gaussians seem to provide much more significant speed boost. }


\officialreply{As the reviewer mentioned, these two methods can be run in parallel. We believe the results may be interesting for graphics specialist considering the fact that \textbf{low-power} GPU rendering can only be achieved with increasingly more efficient parallelization. Sorting is intrinsically sequential, and thus greatly complicates the hardware parallelization by requiring techniques like tiling, and to remove the ``popping'' requires significantly more complicated sorting. Weighted sums, on the other hand, eliminates dependencies and works for these low-power platforms.}



% ** Method **

% The proposed method is largely borrowed from the traditional sort-free methods. I think this is acceptable because of the long history of sort-free rendering research in traditional computer graphics, it does negatively affect the novelty of the proposed method slightly.

% \amir{As with Gaussian Splatting itself, researchers are finding that many ``old'' ideas from Computer Graphics can be made much more effective with differentiable rendering and machine learning techniques. We believe this paper shows that the OIT idea can be similarly greatly extended.}

% \amir{However, it should be also noted that the problem here is different because, instead of having a combination of opaque and semi-transparent elements in fixed settings, all 3DGS elements have intrinsic transparency and all parameters are learned according to rendering results, enabling new ideas like learned view-dependent opacity.}

% \amir{In this regard, another interesting and unexpected finding is that with machine learning it was possible to find that linear weights (LC-WSR), which are less intuitive than OIT exponential weights, not only work well, but in fact produce the best PSNR results!}

% \reply{Thanks. The novelty is the learnable parameters, which were not part of traditional OIT methods. In the ablation study, the learnable parameters improve the results significantly. We also proposed view dependent opacity which is not a part of traditional OIT.


% \randall{we should discuss the extensions, e.g. LC-WSR, that are not part of OIT and improve results.}}




\officialquestion{The proposed method is largely borrowed from the traditional sort-free methods, which negatively affects the novelty of the proposed method slightly }


\officialreply{This paper shows that the OIT idea can be similarly greatly extended. Instead of having a combination of opaque and semi-transparent elements in fixed settings, all 3DGS elements have intrinsic transparency and all parameters are learned according to rendering results, enabling new ideas like learned view-dependent opacity. Another interesting and unexpected finding is that with machine learning it was possible to find that linear weights (LC-WSR), which are less intuitive than OIT exponential weights, not only work well, but in fact produce the best PSNR results.}



** Experiments**

% \amir{Remove?} As mentioned above, the improvement on standard desktop GPU is rather insignificant. 

% Since sort-free rendering is essentially an approximation of the sort-based rendering, it might not be a good idea to choose this method for such a small improvement while there is a possibility of very bad performance on some scenes.

% \amir{Those are improvements for a specific GPU implementation, meant to show some advantages with current GPU hardware. We also believe approaches like WSR may be important for future GPU hardware design discussions, since sort-free methods are much easier and cheaper to parallelize, and thus can be much more efficient.}

% Continuing from the last point, sort-free approximations are usually inaccurate on small and thin structures. For example, I noticed that the proposed method on the bicycle scene in MipNeRF-360 dataset is somewhat lower than the original 3DGS method. This scene contains very thin and fine structures on the bicycle which could be a better illustration of whether the proposed method suffers from similar artifacts like the traditional methods.

% \amir{This is indeed what is expected, and the authors considered that the method would be strongly limited to some specific object shapes and scene types. However, it was found that with machine learning it was possible to get increasingly better results in more scenes.}

% \amir{We do not claim that the proposed method will work for all cases, and recognize that it is weakest for large variations of scene depths and viewing distances. At the same time, we found it much more effective than conventional OIT, and leave it to readers to evaluate if it would be sufficient for their specific applications (e-commerce, product catalogs, etc.}



% Despite the significant rendering speed improvement on the edge devices, the paper lacks a detailed explanation of how the edge device running out of resources leads to such a big decrease in rendering speed.

% \amir{Unfortunately it can be difficult to pinpoint the sources of inefficiency in complex GPUs. To the best of our knowledge this is caused by sudden changes to many more cache misses. We added a comment about this to the paper.}


\officialquestion{Explain how the edge device running out of resources leads to such a big decrease in rendering speed.}


\officialreply{Our implementation of 3DGS appears to be hitting some sort of GPU bottleneck when rendering scenes with a large number of sorted Gaussians. Unfortunately it can be difficult to pinpoint the sources of inefficiency in complex GPUs. To the best of our knowledge, this is caused by sudden changes to many more cache misses.  We suspect that this bottleneck could be addressed with in-depth analysis and GPU specific optimizations, however, this would make our reference implementation less faithful to the original 3DGS implementation. We note that our method appears to be avoid this bottleneck in its simplicity. We added a comment about this to the paper.}


\subsection{Questions}

% Can the authors provide some qualitative results on the Bicycle scene?

% \reply{I need to run more videos on the bicyle scenes}


\officialquestion{Sort-free approximations are usually inaccurate on small and thin structures. Can the authors provide some qualitative results on the Bicycle scene?}


\officialreply{We conducted the suggested experiment to provide additional rendering results on the challenging Bicycle scene, which contains many small and thin structures. The results demonstrate that our method still achieves plausible outcomes in these areas, such as the bicycle spokes. The video can be accessed at: \url{https://anonymous20241121.github.io/sort_free_gs/bicycle.mp4}}



% Can the authors provide some videos showing the removal of the popping effect?

% \amir{We created a video with the well-known scene "Garden" and table reflections where the ``popping'' is easiest to see.}

% \reply{\qiqi{Video demo}}


\officialquestion{Can the authors provide some videos showing the removal of the popping effect?}


\officialreply{We created a video featuring the well-known "Garden" scene, where the "popping" artifacts are most noticeable. Compared to 3DGS, our method successfully eliminates these artifacts by removing the sorting step. The video can be accessed at: \url{https://anonymous20241121.github.io/sort_free_gs/pop.mp4}}


% Can the authors show some failure cases of the proposed approximation?

% \amir{One type of failure that is easy to identify visually is apparent transparency of dark objects when in front of very light background. However, this is something that can be detected with differentiable rendering, and thus can be attributed to suboptimal training.}

% \amir{The question of what cannot be fixed even with better training is much harder to answer, and should be further researched.}

% \reply{\qiqi{More failure case. Bicycle, it can be improved by training or blabla}}




\officialquestion{Can the authors show some failure cases of the proposed approximation?}


\officialreply{One type of failure that is easily identifiable visually is the apparent transparency of dark objects when placed in front of a very light background. However, this issue could be detected with differentiable rendering and can thus be attributed to suboptimal training. In the supplementary material, we have provided a visual example and included a discussion of these failure cases.}


% I really want to give a positive rating to this paper, because I know it is very difficult to make a sort-free rendering to achieve the same quality as the sort-based version. However, the marginal speed improvement diminishes the significance of this paper. Furthermore, I hope the authors can demonstrate some failure cases of such approximation methods, as they are quite common in traditional sort-free algorithms. Doing this could give the reader a more comprehensive understanding of the proposed method.

% \amir{We hope the shared videos can show that the proposed approach has some limitations, but at the same time view are surprisingly good considering its simplicity. We also want to show that although 3DGS sorting may seem inevitable, machine learning can enable it to be replaced.}

% \reply{Thanks}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Fourth Reviewer
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Reviewer : ``uk93''}

% \subsection{Weaknesses}

% This work is of quite a high quality. I do not see any specific weaknesses in the methodology or the experimental results. There is one specific minor weakness in the experimental section wherein I would like further information on the memory requirements of the proposed method. I detail the exact question I have in the "Questions" section below. One final minor issue is the presence of minor grammar errors in the text as I mention in the "Questions" section below.

% \reply{This is addressed in the reply to the question below.}

\subsection{Questions}

% In section 4.3 the authors reveal that view-dependent opacity is obtained by the addition of a new set of spherical harmonics related to the depth weighting introduced by the authors. In the experimental section, the authors show that this doesn't impact memory usage during rendering and a rationale given in the removal of the sorting step and the potential reduction in the number of Gaussians. However, this appears to be referring to instantaneous memory requirements. How does the introduction of the new set of spherical harmonics for each Gaussian affect post-training storage requirements of the radiance field? Is a greater storage footprint needed for the radiance fields produced by the proposed methods?

% \amir{As mentioned before, during rendering there is no overhead because color data needs to be stored as RGBARGBA..., and similarly SIMD instructions operate on vectors of dimension 4. For general storing of the splatting elements, it will indeed increase the footprint because the number of spherical harmonics coefficient values increases from 3 top 4. In this regard, it should be noted that many authors identified spherical harmonic coefficients as the set of parameters that are easiest to compress or prune. We confirmed that in our own experiments, for example, limiting the number of opacity spherical harmonic coefficients. Nevertheless, we decided that compression and data reduction should be outside the scope of the paper, which should be mostly about introducing the WSR approach for mobile devices.}

% \reply{RGB RGBA, easy to compress} 


\officialquestion{How does the introduction of the new set of spherical harmonics for each Gaussian affect post-training storage requirements of the radiance field? Is a greater storage footprint needed for the radiance fields produced by the proposed methods?}


\officialreply{In Table 3, we reported the runtime memory. In the GPU graphic pipeline, the spherical harmonics data needs to be stored as RGBARGBA$\cdots$ instead of RGBRGB$\cdots$, and similarly SIMD instructions operate on vectors of dimension 4. We exploit this fact by using the alpha memory position to create view-dependent opacity, which does not increase the amount of memory and vector operations. For general storing of the splatting elements, it indeed increases the footprint per Gaussians because the number of spherical harmonics coefficient values increases from 3 to 4. We update the Table caption as well as the corresponding part in the experiment section in the revised version. }



\officialquestion{Minor grammar errors}


\officialreply{Thanks for finding those typos, They have all been fixed in the latest version}

% Line 53 "maintain rendering differentiable" should be "maintain rendering differentiability".

% Line 141 "Chris Wyman provide a good survey on these methods" should be "Chris Wyman provides a good survey on these methods"

% Line 273, "However, DIR-WSR does not work well for the complex scenes, " should be "However, DIR-WSR does not work well for complex scenes, "

% \reply{\randall{I believe several of these have been addressed in the arXiv version}}

% Line 307 ends with an additional full stop.

% \amir{Thanks for finding those typos, They have all been fixed in the latest version.}


